Distributional Probabilistic Model Checking

Probabilistic model checking can provide formal guarantees on the behavior of stochastic models relating to a wide range of quantitative properties, such as runtime, energy consumption or cost. But decision making is typically with respect to the expected value of these quantities, which can mask important aspects of the full probability distribution such as the possibility of high-risk, low-probability events or multimodalities. We propose a distributional extension of probabilistic model checking, applicable to discrete-time Markov chains (DTMCs) and Markov decision processes (MDPs). We formulate distributional queries, which can reason about a variety of distributional measures, such as variance, value-at-risk or conditional value-at-risk, for the accumulation of reward until a co-safe linear temporal logic formula is satisfied. For DTMCs, we propose a method to compute the full distribution to an arbitrary level of precision, based on a graph analysis and forward analysis of the model. For MDPs, we approximate the optimal policy with respect to expected value or conditional value-at-risk using distributional value iteration. We implement our techniques and investigate their performance and scalability across a range of benchmark models. Experimental results demonstrate that our techniques can be successfully applied to check various distributional properties of large probabilistic models.

==> 5a_table.tex <==

% \setlength{\tabcolsep}{0.3em} % for the horizontal padding
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[t]
\caption{Experimental results comparing different methods.}
\label{tab:results}
\centering
% \scriptsize
\begin{tabular}{@{}ll|c|c|cccc@{}}
\toprule
 % &  &  &  & \multicolumn{4}{c}{Metrics} \\ \cmidrule(l){5-8} 
\multicolumn{1}{c}{Model} & \multicolumn{1}{c|}{Method} & (Prod.) MDP & Time (s) & $\exp$ & $\CVaR{\alpha}$ & $\VaR{\alpha}$ & $\var$ \\ \midrule
\multirow{4}{*}{Betting Game} & VI & 891 & 0.03 & 61.9 & - & - & - \\
 & VI+DTMC & 891 & 0.03 & 61.9 & 98.0 & 87.0 & 886.8 \\
 & risk-neutral DVI & 891 & 0.25 & \textbf{61.9} & 98.0 & 87.0 & 886.8 \\
 & risk-sensitive DVI & 89,991 & 35.90 & 85.3 & \textbf{92.2} & 88.0 & 55.9 \\ \midrule
\multirow{4}{*}{DS Treasure} & VI & 1,222 & 0.02 & 359.3 & - & - & - \\
 & VI+DTMC & 1,222 & 0.02 & 359.3 & 473.0 & 425.0 & 7,311.8 \\
 & risk-neutral DVI & 1,222 & 0.47 & \textbf{359.3} & 474.6 & 424.0 & 7,351.9 \\
 & risk-sensitive DVI & 123,422 & 72.44 & 370.1 & \textbf{458.6} & 424.0 & 4,405.7 \\ \midrule
\multirow{4}{*}{Obstacle 150} & VI & 22,500 & 0.79 & 402.8 & - & - & - \\
 & VI+DTMC & 22,500 & 1,839.00 & 402.8 & 470.0 & 433.0 & 2,018.6 \\
 & risk-neutral DVI & 22,500 & 96.59 & \textbf{402.7} & 479.2 & 441.0 & 2,702.8 \\
 & risk-sensitive DVI & 2,272,500 & 15,051.10 & 402.9 & \textbf{478.4} & 441.0 & 2,641.4 \\ \midrule
\multirow{4}{*}{UAV} & VI & 16,508 & 0.34 & 124.1 & - & - & - \\
 & VI+DTMC & 16,508 & 0.51 & 124.1 & 169.6 & 130.0 & 1,433.5 \\
 & risk-neutral DVI & 16,508 & 3.59 & \textbf{123.8} & 168.8 & 132.5 & 1,346.8 \\
 & risk-sensitive DVI & 1,667,308 & 2,365.79 & 134.9 & \textbf{169.1} & 130.0 & 933.2 \\ \midrule
\multirow{4}{*}{Energy 15} & VI & 25,819 & 9.72 & 184.3 & - & - & - \\
 & VI+DTMC & 25,819 & 260.76 & 184.3 & 383.8 & 339.0 & 10,635.2 \\
 & risk-neutral DVI & 25,819 & 107.63 & \textbf{184.0} & 382.0 & 340.0 & 10,525.7 \\
 & risk-sensitive DVI & 1,316,769 & 9,384.01 & 184.6 & \textbf{380.9} & 340.0 & 10,419.7 \\ \bottomrule
\end{tabular}
\end{table}

% {for obstacle 150, cvar value of 478.4 is approximate, dtmc computed value (closer to true) is 469}

